Asking More Informative Questions for Grounded Retrieval

When a model is trying to gather information in an interactive setting, it benefits from asking informative questions. However, in the case of a grounded multi-turn image identification task, previous studies have been constrained to polar yes/no questions, limiting how much information the model can gain in a single turn. We present an approach that formulates more informative, open-ended questions. In doing so, we discover that off-the-shelf visual question answering (VQA) models often make presupposition errors, which standard information gain question selection methods fail to account for. To address this issue, we propose a method that can incorporate presupposition handling into both question selection and belief updates. Specifically, we use a two-stage process, where the model first filters out images which are irrelevant to a given question, then updates its beliefs about which image the user intends. Through self-play and human evaluations, we show that our method is successful in asking informative open-ended questions, increasing accuracy over the past state-of-the-art by 14%, while resulting in 48% more efficient games in human evaluations.

==> sections/notes.tex <==
- talk about information gain objective and how to ask more informative questions

- include presupposition in figure
- include question decomposition in high-level figure
- make sure figure is consistent with text
- find a way to include posteriors to show the updates
- use less images and add actual captions/questions

- 4.3 reword "response model"
- move 4.3 to the self-play section
- Section 3 describe as two-turn setting


faq
- blip2
- fair comparison?
- why only human eval for two settings?
- other datasets?
- why don't use clip

Appendix
- IsA question generation
- prompt for gpt
- mturk evaluations -- discuss QUALS!!!
- sample games

- include details about pilot study?

- maybe include hard vs soft probabilities?
The number of questions per caption $j$ ranges from 2 to 7, with an average of 3.41

- check figures
